Search for a scalar partner of the top quark in the jets plus missing transverse momentum final state at $\sqrt{s}$=13 TeV with the ATLAS detector

A search for pair production of a scalar partner of the top quark in events with four or more jets plus missing transverse momentum is presented. An analysis of 36.1 fb$^{-1}$ of $\sqrt{s}$=13 TeV proton-proton collisions collected using the ATLAS detector at the LHC yields no significant excess over the expected Standard Model background. To interpret the results a simplified supersymmetric model is used where the top squark is assumed to decay via $\tilde{t}_1 \rightarrow t^{(*)} \tilde\chi^0_1$ and $\tilde{t}_1\rightarrow b\tilde\chi^\pm_1 \rightarrow b W^{(*)} \tilde\chi^0_1$, where $\tilde\chi^0_1$ ($\chi^\pm_1$) denotes the lightest neutralino (chargino). Exclusion limits are placed in terms of the top-squark and neutralino masses. Assuming a branching ratio of 100% to $t \tilde\chi^0_1$, top-squark masses in the range 450-950 GeV are excluded for $\tilde\chi^0_1$ masses below 160 GeV. In the case where $m_{\tilde{t}_1}\sim m_t+m_{\tilde\chi^0_1}$, top-squark masses in the range 235-590 GeV are excluded.

==> SRAcutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow for SRA for a signal model with top squark pair production in the case where both top squarks decay via $\stop\to t^{(*)} \ninoone$ with $m(\stop,\ninoone)=$ (800,1) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV. }
\begin{center}
\scriptsize

\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 198000 & 1022.85015869 &   \\ 
Derivation Skim & 193641 & 1006 & 0.98 \\ 
No bad jets & 191294 & 994 & 0.97 \\ 
Cosmic muon cut & 189048 & 982 & 0.96 \\ 
No bad muons & 188859 & 981 & 0.96 \\ 
Lepton veto & 111953 & 582 & 0.57 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 108694 & 564 & 0.55 \\ 
\ptmisstrk $>$ 30 GeV & 104626 & 543 & 0.53 \\ 
\nBJet $\geq$ 1 & 96206 & 500 & 0.49 \\ 
\met $>$ 250 GeV & 77152 & 401 & 0.39 \\ 
\dphimettrk$<1/3\pi$ & 72647 & 377 & 0.37 \\ 
\dphijetthreemet $>$ 0.4 & 67270 & 349 & 0.34 \\ 
\ptone $>$ 80 GeV & 65170 & 338 & 0.33 \\ 
\ptthree $>$ 40 GeV & 57955 & 302 & 0.3 \\ 
Pass \met\ Trigger & 57954 & 302 & 0.3 \\ 
\mantikttwelvezero $>$ 120 GeV & 49511 & 257 & 0.25 \\ 
\hline
SRA-TT & & \\ 
\mantikttwelveone $>$ 120 GeV & 15242 & 79.5 & 0.078 \\ 
\met $>$ 400 GeV & 10709 & 55.9 & 0.055 \\ 
\mantikteightzero $>$ 60 GeV & 10022 & 52.3 & 0.051 \\ 
\mtbmin $>$ 200 GeV & 8724 & 45.2 & 0.044 \\ 
Tau Veto & 7891 & 41 & 0.04 \\ 
\drbjetbjet $>$ 1 & 6816 & 35.2 & 0.034 \\ 
\mttwo $>$ 400 GeV & 6236 & 32.1 & 0.031 \\ 
\nBJet $\geq$ 2 & 4120 & 21.2 & 0.021 \\ 
\hline
SRA-TW & & \\ 
\mantikttwelveone $<$ 120 GeV & 33835 & 175 & 0.17 \\ 
\mantikttwelveone $>$ 60 GeV & 13584 & 70.4 & 0.069 \\ 
\met $>$ 500 GeV & 6564 & 34.2 & 0.033 \\ 
\mantikteightzero $>$ 60 GeV & 6155 & 32.1 & 0.031 \\ 
\mtbmin $>$ 200 GeV & 5401 & 28 & 0.027 \\ 
Tau Veto & 4849 & 25.1 & 0.025 \\ 
\mttwo $>$ 400 GeV & 4655 & 24.1 & 0.024 \\ 
\nBJet $\geq$ 2 & 2778 & 14.5 & 0.014 \\ 
\hline
SRA-T0 & & \\ 
\mantikttwelveone $<$ 60 GeV & 20251 & 105.4 & 0.1 \\ 
\mantikteightzero $>$ 60 GeV & 17623 & 91.4 & 0.089 \\ 
\met $>$ 550 GeV & 8655 & 44.9 & 0.044 \\ 
\mtbmin $>$ 200 GeV & 7699 & 39.7 & 0.039 \\ 
Tau Veto & 6946 & 36 & 0.035 \\ 
\mttwo $>$ 500 GeV & 6068 & 31.4 & 0.031 \\ 
\nBJet $\geq$ 2 & 3607 & 18.8 & 0.018 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRA}
\end{table}


==> SRBcutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow SRB for a signal model with top squark pair production in the case where both top squarks decay via $\stop\to t^{(*)} \ninoone$ with $m(\stop,\ninoone)=$ (600,300) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV. }
\begin{center}
\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 200000 & 6303.02392578 &   \\ 
Derivation Skim & 179739 & 5680 & 0.9 \\ 
No bad jets & 177598 & 5620 & 0.89 \\ 
Cosmic muon cut & 175640 & 5550 & 0.88 \\ 
No bad muons & 175519 & 5550 & 0.88 \\ 
Lepton veto & 100787 & 3190 & 0.51 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 98693 & 3120 & 0.5 \\ 
\ptmisstrk $>$ 30 GeV & 89253 & 2820 & 0.45 \\ 
\nBJet $\geq$ 1 & 81668 & 2600 & 0.41 \\ 
\met $>$ 250 GeV & 36204 & 1162 & 0.18 \\ 
\dphimettrk$<1/3\pi$ & 34344 & 1102 & 0.17 \\ 
\dphijetthreemet $>$ 0.4 & 31219 & 1000 & 0.16 \\ 
\ptone $>$ 80 GeV & 27782 & 894 & 0.14 \\ 
\ptthree $>$ 40 GeV & 23902 & 773 & 0.12 \\ 
Pass \met\ Trigger & 23901 & 773 & 0.12 \\ 
\mantikttwelvezero $>$ 120 GeV & 15900 & 512 & 0.081 \\ 
\hline
SRB-TT & & \\ 
\mantikttwelveone $>$ 120 GeV & 2639 & 86 & 0.014 \\ 
\drbjetbjet $>$ 1.2 & 2200 & 72 & 0.011 \\ 
\mtbmax $>$ 200 GeV & 1871 & 61 & 0.0097 \\ 
\mtbmin $>$ 200 GeV & 1215 & 39 & 0.0062 \\ 
Tau Veto & 1019 & 32 & 0.0052 \\ 
\nBJet $\geq$ 2 & 610 & 19.8 & 0.0031 \\ 
\hline
SRB-TW & & \\ 
\mantikttwelveone $<$ 120 GeV & 13243 & 424 & 0.067 \\ 
\mantikttwelveone $>$ 60 GeV & 4474 & 143 & 0.023 \\ 
\drbjetbjet $>$ 1.2 & 3608 & 115 & 0.018 \\ 
\mtbmax $>$ 200 GeV & 2971 & 95 & 0.015 \\ 
\mtbmin $>$ 200 GeV & 1874 & 58 & 0.0093 \\ 
Tau Veto & 1558 & 49 & 0.0078 \\ 
\nBJet $\geq$ 2 & 785 & 25.3 & 0.004 \\ 
\hline
SRB-T0 & & \\ 
\mantikttwelveone $<$ 60 GeV & 8769 & 281 & 0.045 \\ 
\mtbmin $>$ 200 GeV & 5093 & 160 & 0.026 \\ 
\drbjetbjet $>$ 1.2 & 3472 & 109 & 0.017 \\ 
\mtbmax $>$ 200 GeV & 3378 & 106 & 0.017 \\ 
\met $>$ 250 GeV & 3378 & 106 & 0.017 \\ 
Tau Veto & 2809 & 88 & 0.014 \\ 
\nBJet $\geq$ 2 & 1340 & 43 & 0.007 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRB}
\end{table}


==> SRC12cutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow for SRC1 and SRC2 for a signal model with top squark pair production in the case where both top squarks decay via $\stop\to t^{(*)} \ninoone$ with $m(\stop,\ninoone)=$ (250,77) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV. }
\begin{center}
\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 566000 & 131132.47&   \\ 
Derivation Skim & 463692 & 108390 & 0.83 \\ 
No bad jets & 458395 & 107100 & 0.82 \\ 
Cosmic muon cut & 452204 & 105600 & 0.81 \\ 
No bad muons & 451917 & 105570 & 0.81 \\ 
Lepton veto & 171980 & 40160 & 0.31 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 163616 & 38100 & 0.29 \\ 
\ptmisstrk $>$ 30 GeV & 137883 & 32150 & 0.25 \\ 
\nBJet $\geq$ 1 & 124536 & 29290 & 0.22 \\ 
\met $>$ 250 GeV & 11921 & 2840 & 0.022 \\ 
\dphimettrk$<1/3\pi$ & 10302 & 2450 & 0.019 \\ 
\dphijettwomet $>$ 0.4 & 7574 & 1810 & 0.014 \\ 
\ptone $>$ 80 GeV & 6737 & 1610 & 0.012 \\ 
\ptthree $>$ 40 GeV & 5561 & 1340 & 0.01 \\ 
Pass \met\ Trigger & 5560 & 1340 & 0.01 \\ 
\nBJetS $\geq$ 1 & 4622 & 1110 & 0.0085 \\ 
\nJetS $\geq$ 5 & 1206 & 270 & 0.0021 \\ 
\pTSBZero $>$ 40 & 1134 & 253 & 0.0019 \\ 
\mS $>$ 300 & 962 & 214 & 0.0016 \\ 
\dPhiISRMET $>$ 3.00 & 426 & 95 & 0.00073 \\ 
\pTISR $>$ 400 & 425 & 95 & 0.00072 \\ 
\pTSFour $>$ 50 & 307 & 68 & 0.00052 \\ 
\hline
SRC1 & & \\ 
0.30 $\leq$ \rISR $\leq$ 0.40 & 152 & 33 & 0.00026 \\ 
\hline
SRC2 & & \\ 
0.40 $\leq$ \rISR $\leq$ 0.50 & 82 & 18 & 0.00014 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRC12}
\end{table}


==> SRC35cutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow for SRC3, SRC4, and SRC5 for a signal model with top squark pair production in the case where both top squarks decay via $\stop\to t^{(*)} \ninoone$ with $m(\stop,\ninoone)=$ (500,327) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV. }
\begin{center}
\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 200000 & 7227.81 &   \\ 
Derivation Skim & 174497 & 6350 & 0.88 \\ 
No bad jets & 172301 & 6270 & 0.87 \\ 
Cosmic muon cut & 170225 & 6200 & 0.86 \\ 
No bad muons & 170116 & 6190 & 0.86 \\ 
Lepton veto & 86653 & 3180 & 0.44 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 85311 & 3130 & 0.43 \\ 
\ptmisstrk $>$ 30 GeV & 73340 & 2690 & 0.37 \\ 
\nBJet $\geq$ 1 & 66620 & 2470 & 0.34 \\ 
\met $>$ 250 GeV & 17782 & 649 & 0.09 \\ 
\dphimettrk$<1/3\pi$ & 16108 & 589 & 0.082 \\ 
\dphijettwomet $>$ 0.4 & 12419 & 459 & 0.064 \\ 
\ptone $>$ 80 GeV & 11132 & 413 & 0.057 \\ 
\ptthree $>$ 40 GeV & 10292 & 382 & 0.053 \\ 
Pass \met\ Trigger & 10292 & 382 & 0.053 \\ 
\nBJetS $\geq$ 1 & 8769 & 327 & 0.045 \\ 
\nJetS $\geq$ 5 & 3094 & 111 & 0.015 \\ 
\pTSBZero $>$ 40 & 2733 & 98 & 0.014 \\ 
\mS $>$ 300 & 2296 & 82 & 0.011 \\ 
\dPhiISRMET $>$ 3.00 & 1295 & 46 & 0.0064 \\ 
\pTISR $>$ 400 & 1284 & 45 & 0.0063 \\ 
\pTSFour $>$ 50 & 518 & 18.8 & 0.0026 \\ 
\hline
SRC3 & & \\ 
0.50 $\leq$ \rISR $\leq$ 0.60 & 212 & 7.6 & 0.001 \\ 
\hline
SRC4 & & \\ 
0.60 $\leq$ \rISR $\leq$ 0.70 & 237 & 8.6 & 0.0012 \\ 
\hline
SRC5 & & \\ 
0.70 $\leq$ \rISR $\leq$ 0.80 & 28 & 1 & 0.00013 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRC35}
\end{table}


==> SRDhighcutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow for SRD-high for a signal model with bottom squark pair production in the case where both bottom squarks decay via $b\chinoonepm\ra bW^{(*)}\ninoone$, with $m(\chinoonepm)-m(\ninoone) = 1$ GeV with $m(\stop,\chinoonepm)=$ (800,100) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV.}
\begin{center}
\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 10000 & 1557.42 &   \\ 
Derivation Skim & 9728 & 1540 & 0.99 \\ 
No bad jets & 9618 & 1530 & 0.98 \\ 
Cosmic muon cut & 9544 & 1520 & 0.97 \\ 
No bad muons & 9536 & 1510 & 0.97 \\ 
Lepton veto & 9294 & 1470 & 0.95 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 6301 & 1000 & 0.64 \\ 
\ptmisstrk $>$ 30 GeV & 5890 & 930 & 0.6 \\ 
\nBJet $\geq$ 1 & 5340 & 830 & 0.54 \\ 
\met $>$ 250 GeV & 4124 & 650 & 0.41 \\ 
\dphimettrk$<1/3\pi$ & 3653 & 570 & 0.37 \\ 
\dphijetthreemet $>$ 0.4 & 3293 & 513 & 0.33 \\ 
\ptone $>$ 80 GeV & 3175 & 496 & 0.32 \\ 
\ptthree $>$ 40 GeV & 1836 & 293 & 0.19 \\ 
Pass \met\ Trigger & 1836 & 293 & 0.19 \\ 
$N_{\mathrm{jets}}$ $\geq$ 5 & 1468 & 233 & 0.15 \\ 
\ptone $>$ 150 GeV & 1216 & 195 & 0.13 \\ 
\ptthree $>$ 80 GeV & 542 & 90 & 0.058 \\ 
\ptfour $>$ 60 GeV & 267 & 45 & 0.029 \\ 
\mtbmin $>$ 350 GeV & 203 & 34 & 0.022 \\ 
\mtbmax $>$ 450 GeV & 171 & 28 & 0.018 \\ 
\nBJet $\geq$ 2 & 97 & 15 & 0.0097 \\ 
\met $>$ 250 GeV & 97 & 15 & 0.0097 \\ 
\drbjetbjet $>$ 0.8 & 89 & 13 & 0.0089 \\ 
\ptbzero+\ptbone $>$ 400 GeV & 75 & 11 & 0.0074 \\ 
Tau Veto & 69 & 10 & 0.0068 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRDhigh}
\end{table}


==> SRDlowcutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow for SRD-low for a signal model with bottom squark pair production in the case where both bottom squarks decay via $b\chinoonepm\ra bW^{(*)}\ninoone$, with $m(\chinoonepm)-m(\ninoone) = 1$ GeV witht $m(\stop,\chinoonepm)=$ (600,200) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV.}
\begin{center}
\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 176000 & 66256.85 &   \\ 
Derivation Skim & 139998 & 53160 & 0.8 \\ 
No bad jets & 138331 & 52500 & 0.79 \\ 
Cosmic muon cut & 137213 & 52090 & 0.79 \\ 
No bad muons & 137144 & 52070 & 0.79 \\ 
Lepton veto & 133236 & 50570 & 0.76 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 74038 & 28200 & 0.43 \\ 
\ptmisstrk $>$ 30 GeV & 61728 & 23600 & 0.36 \\ 
\nBJet $\geq$ 1 & 57761 & 22130 & 0.33 \\ 
\met $>$ 250 GeV & 19965 & 7770 & 0.12 \\ 
\dphimettrk$<1/3\pi$ & 18834 & 7320 & 0.11 \\ 
\dphijetthreemet $>$ 0.4 & 17017 & 6610 & 0.1 \\ 
\ptone $>$ 80 GeV & 14125 & 5560 & 0.084 \\ 
\ptthree $>$ 40 GeV & 7427 & 3020 & 0.046 \\ 
Pass \met\ Trigger & 7427 & 3020 & 0.046 \\ 
$N_{\mathrm{jets}}$ $\geq$ 5 & 5799 & 2340 & 0.035 \\ 
\nBJet $\geq$ 2 & 3732 & 1520 & 0.023 \\ 
\met $>$ 250 GeV & 3732 & 1520 & 0.023 \\ 
\mtbmin $>$ 250 GeV & 1942 & 780 & 0.012 \\ 
\mtbmax $>$ 300 GeV & 1462 & 590 & 0.0088 \\ 
\drbjetbjet $>$ 0.8 & 1326 & 530 & 0.008 \\ 
\ptone $>$ 150 GeV & 672 & 270 & 0.0041 \\ 
\ptthree $>$ 100 GeV & 252 & 102 & 0.0015 \\ 
\ptfour $>$ 60 GeV & 141 & 56 & 0.00085 \\ 
\ptbzero+\ptbone $>$ 300 GeV & 105 & 41 & 0.00062 \\ 
Tau Veto & 96 & 37 & 0.00057 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRDlow}
\end{table}


==> SREcutflowtable.tex <==
\begin{table}[htpb]
\caption{Cutflow for SRE for a signal model with gluino pair production in the case where both gluinos decay via $\gluino\to t\stop\to t\ninoone+$soft and $\Delta m(\stop,\ninoone)=5\GeV$ with $m(\gluino,\stop)=$ (1700,400) GeV. An integrated luminosity of 36.1 \ifb\ is assumed when calculating the weighted yields.  For the derivation skim at least one of the following four criteria is required: \HT\ $>$ 150 GeV; at least one loose electron with \pt\ $>$ 100 GeV or at least two loose electrons with \pt\ $>$ 20 GeV; at least one muon with \pt\ $>$ 100 GeV or at least two muons with \pt\ $>$ 20 GeV; or at least one photon with \pt\ $>$ 100 GeV  or at least two photons with \pt\ $>$ 50 GeV. }
\begin{center}
\begin{tabular}{l||c|c|c}
\hline \hline
Cut & Unweighted Yield & Weighted Yield & Efficiency*Acceptance \\ 
\hline
Total & 100000 & 169.786605835 &   \\ 
Derivation Skim & 99697 & 172.1 & 1.0 \\ 
No bad jets & 98957 & 170.8 & 1.0 \\ 
Cosmic muon cut & 97334 & 168 & 0.99 \\ 
No bad muons & 97151 & 167.7 & 0.99 \\ 
Lepton veto & 58969 & 101.8 & 0.6 \\ 
$N_{\mathrm{jets}}$ $\geq$ 4 & 56406 & 97.1 & 0.57 \\ 
\ptmisstrk $>$ 30 GeV & 55569 & 95.7 & 0.56 \\ 
\nBJet $\geq$ 1 & 49816 & 85.5 & 0.5 \\ 
\met $>$ 250 GeV & 46437 & 79.7 & 0.47 \\ 
\dphimettrk$<1/3\pi$ & 42890 & 73.6 & 0.43 \\ 
\dphijetthreemet $>$ 0.4 & 38881 & 66.6 & 0.39 \\ 
\ptone $>$ 80 GeV & 38461 & 65.9 & 0.39 \\ 
\ptthree $>$ 40 GeV & 32792 & 56.3 & 0.33 \\ 
Pass \met\ Trigger & 32792 & 56.3 & 0.33 \\ 
\met $>$ 550 GeV & 26309 & 45.2 & 0.27 \\ 
\mantikteightzero $>$ 120 GeV & 22609 & 38.8 & 0.23 \\ 
\mantikteightone $>$ 80 GeV & 13263 & 22.8 & 0.13 \\ 
\HT $>$ 800 GeV & 13254 & 22.7 & 0.13 \\ 
\htsig $>$ 18 $\sqrt{\GeV}$ & 10827 & 18.6 & 0.11 \\ 
\mtbmin $>$ 200 GeV & 9759 & 16.6 & 0.098 \\ 
\nBJet $\geq$ 2 & 5563 & 9.4 & 0.056 \\ 
\hline\hline
\end{tabular}
\end{center}
\label{tab:cutflowSRE}
\end{table}

